Convolutional Conditional Neural Processes

We introduce the Convolutional Conditional Neural Process (ConvCNP), a new member of the Neural Process family that models translation equivariance in the data. Translation equivariance is an important inductive bias for many learning problems including time series modelling, spatial data, and images. The model embeds data sets into an infinite-dimensional function space as opposed to a finite-dimensional vector space. To formalize this notion, we extend the theory of neural representations of sets to include functional representations, and demonstrate that any translation-equivariant embedding can be represented using a convolutional deep set. We evaluate ConvCNPs in several settings, demonstrating that they achieve state-of-the-art performance compared to existing NPs. We demonstrate that building in translation equivariance enables zero-shot generalization to challenging, out-of-domain tasks.

==> figures/algorithms/algorithm_and_diagram.tex <==
\begin{figure}[t]
    \hfill
    \begin{subfigure}{0.52\linewidth}
        \begin{algorithm}[H]
            \SetKwInOut{Input}{require\!}
            \SetKwInOut{Output}{return}
            \Input{ $\rho = (\text{CNN}, \psi_\rho)$, $\psi$, density $\gamma$}
            \Input{ context $(\vx_n, y_n)_{n=1}^N$, target $(\vx^\ast_m)_{m=1}^M$}
            \Begin{
                $ \text{lower, upper} \leftarrow \text{range}\!\left( (\vx_n)_{n=1}^N \cup (\vx^\ast_m)_{m=1}^M \right)$\\
                $(\vt_i)_{i=1}^T \leftarrow \text{uniform\_grid(lower, upper} ; \gamma)$\\
                $\vh_i \leftarrow \sum_{n=1}^N \begin{bmatrix} 1 \\ y_n  \end{bmatrix} \psi(\vt_i - \vx_n)$\\
                $\vh^{(1)}_i \leftarrow \vh^{(1)}_i / \vh^{(0)}_i$\\
                $(f_\mu(\vt_i), f_\sigma(\vt_i))_{i=1}^T \leftarrow \textsc{CNN}((\vt_i, \vh_i)_{i=1}^T)$\\
                $\vmu_m \leftarrow \sum_{i=1}^T f_\mu(\vt_i) \psi_\rho(\vx^\ast_m - \vt_i)$\\
                $\vsigma_m \leftarrow \sum_{i=1}^T \exp(f_\sigma(\vt_i)) \psi_\rho(\vx^\ast_m - \vt_i)$\\
                \KwRet{$(\vmu_m, \vsigma_m)_{m=1}^M$}
            }
        \end{algorithm}
        \vspace{-1em}
        \caption{}
        \label{alg:forward_pass_uncountable}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/algorithms/ConvCNP-Diagram2.pdf}
        \caption{}
        \vspace{-1.75em}
        \label{fig:convps_in_practice}
        % Aligning the captions with the [t] option seems to bug out. The \vspace aligns them manually.
    \end{subfigure}
    \hfill
    \setlength{\belowcaptionskip}{-14pt}
    \vspace{-0.5em}
    \caption{(a) Pseudo-code for and (b) illustration of \convcp{} forward pass.}
    ~ % The empty space here is needed for the \hfills to behave appropriately, for some reason. LaTeX...
\end{figure}


==> figures/plasticc/plasticc_fig.tex <==
\begin{figure}[htb]
\centering
     %%% Success cases %%%
     %%%  ConvNP  %%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{figures/plasticc/convnp_gp_success.png}
  \subcaption{\convcp{}}
  \label{fig:plasticc_convnp_gp_success}
\end{subfigure}\hfill
    %%%    GP     %%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{figures/plasticc/gp_success.png}
  \subcaption{GP}
  \label{fig:plasticc_gp_success}
\end{subfigure}\hfill
     %%% Failure cases %%%
     %%%  ConvNP  %%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{figures/plasticc/convnp_gp_failure.png}
  \subcaption{\convcp{}}
  \label{fig:plasticc_convnp_gp_fail}
\end{subfigure}\hfill
     %%%    GP     %%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{figures/plasticc/gp_failure.png}
  \subcaption{GP}
  \label{fig:plasticc_gp_fail}
\end{subfigure}

\caption{Example functions learned by the (left) \convcp{} and (right) expert GP model from \citep{boone2019avocado}. Left two columns compare \convcp{} to the expert model in a successful case of the GP, right two columns compare on a case where the GP has failed to capture both the structure or the uncertainty of the data.}
\label{fig:plasticc_fig}
\end{figure}

==> tables/synth_1d_all.tex <==
\begin{table}[]
\begin{tabular}{llllll}
\hline
              &            & \multicolumn{2}{c}{Exponentiated Quadratic}            & \multicolumn{2}{c}{Weakly Periodic}                    \\ 
Model          & Parameters & \multicolumn{1}{c}{log like} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{log like} & \multicolumn{1}{c}{MSE} \\ \hline
CNP            & 66818      & 0.876 $\pm$ 0.657            & 0.036 $\pm$ 0.162       & -1.098 $\pm$ 0.331           & 0.612 $\pm$ 0.377       \\
\anp{}         & 149250     & 2.576 $\pm$ 0.858            & 0.024 $\pm$ 0.191       & -1.100 $\pm$ 0.398           & 0.534 $\pm$ 0.348       \\
NoConv         & 37         & 1.685 $\pm$ 0.982            & 0.082 $\pm$ 0.256       & -1.183 $\pm$ 0.367           & 0.691 $\pm$ 0.474       \\
SimpleConv     & 6537       & 2.057 $\pm$ 1.074            & 0.091 $\pm$ 0.267       & -1.139 $\pm$ 0.428           & 0.648 $\pm$ 0.443       \\
HourGLassConv  & 6537       & 1.673 $\pm$ 1.116            & 0.072 $\pm$ 0.242       & -1.098 $\pm$ 0.439           & 0.655 $\pm$ 0.449       \\
Unet           & 7209       & 2.279 $\pm$ 1.172            & 0.082 $\pm$ 0.254       & -1.017 $\pm$ 0.368           & 0.654 $\pm$ 0.449       \\
SimpleConvXL   & 40665      & 1.203 $\pm$ 1.072            & 0.082 $\pm$ 0.248       & -0.988 $\pm$ 0.433           & 0.560 $\pm$ 0.406       \\
HourGLassCovXL & 40665      & 2.169 $\pm$ 0.945            & 0.022 $\pm$ 0.162       & -0.372 $\pm$ 0.440           & 0.176 $\pm$ 0.219       \\
UnetXL         & 50617      & 2.934 $\pm$ 0.950            & 0.017 $\pm$ 0.152       & -0.410 $\pm$ 0.398           & 0.196 $\pm$ 0.254       \\ \hline
              &            &                              &                         &                              &                         \\ \hline
              &            & \multicolumn{2}{c}{Mixture EQ With Noise}              & \multicolumn{2}{c}{Matern 5/2}                         \\
Model          & Parameters & \multicolumn{1}{c}{log like} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{log like} & \multicolumn{1}{c}{MSE} \\ \hline
CNP            & 66818      & -1.428 $\pm$ 0.164           & 1.010 $\pm$ 0.299       & -0.780 $\pm$ 0.314           & 0.332 $\pm$ 0.239       \\
ANP            & 149250     & -1.228 $\pm$ 0.286           & 0.827 $\pm$ 0.382       & -0.419 $\pm$ 0.487           & 0.251 $\pm$ 0.281       \\
NoConv         & 37         & 0.072 $\pm$ 0.689            & 0.351 $\pm$ 0.597       & -0.123 $\pm$ 0.573           & 0.332 $\pm$ 0.300       \\
SimpleConv     & 6537       & 0.319 $\pm$ 0.707            & 0.271 $\pm$ 0.516       & 0.366 $\pm$ 0.751            & 0.232 $\pm$ 0.268       \\
HourGLassConv  & 6537       & 0.404 $\pm$ 0.718            & 0.260 $\pm$ 0.504       & 0.329 $\pm$ 0.688            & 0.211 $\pm$ 0.257       \\
Unet           & 7209       & 0.333 $\pm$ 0.700            & 0.266 $\pm$ 0.512       & 0.354 $\pm$ 0.752            & 0.218 $\pm$ 0.262       \\
SimpleConvXL   & 40665      & 0.468 $\pm$ 0.734            & 0.218 $\pm$ 0.454       & 0.124 $\pm$ 0.621            & 0.224 $\pm$ 0.254       \\
HourGLassCovXL & 40665      & 0.453 $\pm$ 0.744            & 0.180 $\pm$ 0.379       & 0.113 $\pm$ 0.618            & 0.176 $\pm$ 0.236       \\
UnetXL         & 50617      & 0.719 $\pm$ 0.766            & 0.157 $\pm$ 0.335       & 0.500 $\pm$ 0.751            & 0.175 $\pm$ 0.237       \\ \hline
              &            &                              &                         &                              &                         \\ \hline
              &            & \multicolumn{2}{c}{Sawtooth}                           &                              &                         \\
Model          & Parameters & \multicolumn{1}{c}{log like} & \multicolumn{1}{c}{MSE} &                              &                         \\ \hline
CNP            & 66818      & -0.161 $\pm$ 0.004           & 0.081 $\pm$ 0.001       &                              &                         \\
ANP            & 149250     & 0.330 $\pm$ 0.416            & 0.052 $\pm$ 0.019       &                              &                         \\
NoConv         & 37         & -3.506 $\pm$ 3.282           & 0.053 $\pm$ 0.016       &                              &                         \\
SimpleConv     & 6537       & 2.205 $\pm$ 0.930            & 0.016 $\pm$ 0.011       &                              &                         \\
HourGLassConv  & 6537       & 1.603 $\pm$ 0.407            & 0.025 $\pm$ 0.009       &                              &                         \\
Unet           & 7209       & 2.142 $\pm$ 0.667            & 0.020 $\pm$ 0.011       &                              &                         \\
SimpleConvXL   & 40665      & 2.053 $\pm$ 0.450            & 0.014 $\pm$ 0.007       &                              &                         \\
HourGLassCovXL & 40665      & 2.476 $\pm$ 0.391            & 0.008 $\pm$ 0.002       &                              &                         \\ 
UnetXL         & 50617      & 2.658 $\pm$ 0.232            & 0.007 $\pm$ 0.002       &                              &                         \\ \hline
\end{tabular}
\end{table}

==> tables/synth_1d_loglik.tex <==
\begin{table}[!htb]
\centering
\caption{Log-likelihood from synthetic 1-dimensional experiments.}
\label{table:synthetic_results}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Model         & 
Params        & 
EQ            & 
Weak Periodic & 
Matern        & 
Sawtooth      \\
%
\midrule
%
CNP                  & 
   66818             & 
  -1.49 $\pm$  3e-3  & 
  -2.00 $\pm$ 2e-3   & 
  -1.61 $\pm$ 1e-3   & 
  -0.51 $\pm$ 1e-5   \\
%
\anp                 & 
   149250            & 
   1.08 $\pm$  4e-3  & 
   -2.01 $\pm$ 2e-3  &  
   0.42 $\pm$ 2e-3   & 
   -0.50 $\pm$ 2e-3  \\
%
\convcp{}            & 
   6537              & 
   1.03 $\pm$  5e-3  & 
   -1.52 $\pm$ 2e-3  &  
   0.51 $\pm$ 4e-3   &  
   4.38 $\pm$ 4e-3   \\
%
\convcp{}XL          & 
   50617                       & 
   \textbf{1.90 $\pm$ 4e-3}    & 
   \textbf{-1.19 $\pm$ 2e-3}   & 
   \textbf{0.81 $\pm$ 4e-3}    & 
   \textbf{6.01 $\pm$ 1e-3}   \\ 
%
\bottomrule
%
\end{tabular}
\end{table}
